UniMPA: A Unified Memory-Prediction-Action Model via Action-Grounded Transition Modeling

Recent advances in Vision-Language-Action (VLA) models have improved robotic manipulation, yet observation-to-action learning remains limited by a fundamental transition realizability gap, manifested in three tightly coupled problems: (i) Transition ambiguity. Visually similar current observations may correspond to different manipulation phases and imply different subsequent transitions. (ii) Prediction--execution mismatch. A visually plausible predicted future observation does not necessarily correspond to a physically realizable transition. (iii) Experience--realization mismatch. A historically executable action pattern may not necessarily realize the intended transition in the current scene and therefore requires context-aware adaptation. Accordingly, we propose UniMPA, a Unified Memory-Prediction-Action model that addresses these problems through a shared action-grounded transition interface. (i) UniMPA introduces Persistent-Selective Future Prediction to resolve transition ambiguity by modeling the intended future state evolution. A persistent latent stream continuously tracks task-level progress, while a transition-critical pixel stream selectively resolves fine-grained interaction changes through memory-grounded prediction. (ii) To assess the physical executability of the anticipated transition, the predicted transition queries a temporal Visual-Action Memory Bank. The bank retrieves historically realized visual-action experience, grounding future prediction in executable evidence. (iii) To adapt executable experience to the current scene, an Action-Visual Memory Bank retrieves visually grounded action prototypes from historical action evolution. Prototype-Biased Flow then shifts the flow source toward a historically supported action manifold for context-aware refinement.

==> Tables/ablation-delta.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation study on the future prediction offset $\Delta$.}}
\label{tab:ablation_future_offset}
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccccc}
\toprule
\textbf{Future Offset $\boldsymbol{\Delta}$}
& \textbf{Spatial}
& \textbf{Object}
& \textbf{Goal}
& \textbf{Long}
& \textbf{Avg.}
\\
\midrule

1
& 98.6 & 99.0 & 97.0 & 91.8 & 96.6
 \\


\textbf{8}
& \textbf{99.6}
& \textbf{99.8}
& \textbf{98.8}
& \textbf{96.0}
& \textbf{98.6}
 \\


16
& 98.2 & 98.6 & 96.4 & 89.8 & 95.8
 \\

\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/ablation-lambda.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation study on the action prior strength $\lambda_p$.}}
\label{tab:ablation_lambda_p}
\setlength{\tabcolsep}{8.5pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|ccccc|cc}
    \toprule
    $\boldsymbol{\lambda_p}$
    & \textbf{Spatial}
    & \textbf{Object}
    & \textbf{Goal}
    & \textbf{Long}
    & \textbf{Avg.}
    & \textbf{RW TSR}
    & \textbf{RW CSR} \\
    \midrule
    
    0
    & 98.4 & 98.8 & 96.6 & 91.0 & 96.2
    & 67.2 & 79.5 \\
    
    0.25
    & 99.0 & 99.2 & 97.8 & 93.8 & 97.5
    & 73.2 & 84.1 \\
    
    \textbf{0.5}
    & \textbf{99.6}
    & \textbf{99.8}
    & \textbf{98.8}
    & \textbf{96.0}
    & \textbf{98.6}
    & \textbf{76.8}
    & \textbf{86.9} \\
    
    1.0
    & 99.2 & 99.4 & 98.0 & 93.8 & 97.6
    & 73.6 & 84.5 \\
    
    2.0
    & 98.4 & 98.8 & 96.8 & 90.6 & 96.2
    & 68.7 & 80.6 \\
    
    \bottomrule
    \end{tabular}%
}
\end{table}

==> Tables/robotwin.tex <==
\begin{table*}[t]
\vspace{-4mm}
\caption{\textbf{Results on RoboTwin 2.0 benchmark~\cite{chen2025robotwin}}. All policies are trained on the Clean setting and evaluated without task-specific adaptation on 22 representative tasks under the \textbf{Randomized (hard) zero-shot} setting, with 100 rollouts per task. Results for all 50 tasks are provided in the Appendix.}
\vspace{-5pt}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.05}
\label{tab:robotwin_random_subset}
\resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccccccccccc}
    \toprule
    Method & Adjust B & Dump BB & Grab R & Move PA & Open L & Place A2B-L & Place A2B-R & Place BB & Place BF & Place CP & Place DS\\

    \midrule

    
    ACT~\textit{[RSS'23]}~\cite{zhao2023act} 
    & 23\% & 1\% & 25\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 1\% & 0\%\\
    
    DP~\textit{[RSS'23]}~\cite{diff} 
    & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\%\\
    
    DP3~\textit{[RSS'24]}~\cite{ze20243d} 
    & 3\% & 53\% & 2\% & 3\% & 7\% & 2\% & 0\% & 1\% & 18\% & 1\% & 0\%\\
    
    $\pi_{0}$~\textit{[RSS'25]}~\cite{pi0} 
    & 56\% & 24\% & 80\% & 22\% & 46\% & 1\% & 6\% & 4\% & 4\% & 45\% & 0\%\\

    RDT~\textit{[ICLR'25]}~\cite{liu2024rdt} 
    & 75\% & 32\% & 43\% & 11\% & 32\% & 1\% & 1\% & 2\% & 27\% & 17\% & 4\%\\

    UP-VLA~\textit{[ICML'25]}~\cite{zhang2025up} 
    & 17\% & 35\% & 28\% & 13\% & 21\% & 4\% & 1\% & 20\% & 26\% & 48\% & 0\%\\

    TwinVLA~\textit{[ICLR'26]}~\cite{im2025twinvla}
    & 35\% & 34\% & 22\% & 35\% & 17\% & 5\% & 1\% & 3\% & 13\% & 4\% & 3\%\\

    BagelVLA~\textit{[RSS'26]}~\cite{hu2026bagelvla}
    & 14\% & 51\% & 41\% & 30\% & 37\% & 12\% & 11\% & 29\% & 11\% & 58\% & 0\%\\

    HALO~\textit{[ICML'26]}~\cite{shou2026halo}
    & 9\% & 28\% & 57\% & \textbf{53\%} & 37\% & 8\% & 9\% & 26\% & 37\% & 22\% & 3\%\\

    \midrule
    \rowcolor[HTML]{EFE9F7} 
    \textbf{UniMPA} 
    & \textbf{80\%} & \textbf{62\%} & \textbf{84\%} & 46\% & \textbf{67\%} & \textbf{20\%} & \textbf{14\%} & \textbf{31\%} & \textbf{40\%} & \textbf{75\%} & \textbf{7\%} \\
    \bottomrule

\noalign{\vskip 2pt}

    \toprule
    Method & Place EC & Place Fan & Place OSc & Place OSt & Place PS & Place Shoe & Place St & Rotate ORC & Shake BH & Stamp S & Turn S\\

    \midrule

    
    ACT~\textit{[RSS'23]}~\cite{zhao2023act} 
    & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 6\% & 0\% & 4\% & 0\% & 2\%\\
    
    DP~\textit{[RSS'23]}~\cite{diff} 
    & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 0\% & 18\% & 0\% & 1\%\\
    
    DP3~\textit{[RSS'24]}~\cite{ze20243d} 
    & 1\% & 1\% & 0\% & 0\% & 2\% & 2\% & 3\% & 1\% & 25\% & 0\% & 8\%\\
    
    $\pi_{0}$~\textit{[RSS'25]}~\cite{pi0} 
    & 11\% & 10\% & 0\% & 11\% & 7\% & 6\% & 29\% & 15\% & 51\% & 4\% & 23\%\\

    RDT~\textit{[ICLR'25]}~\cite{liu2024rdt} 
    & 7\% & 2\% & 0\% & 5\% & 6\% & 7\% & 24\% & 5\% & 51\% & 0\% & 15\%\\

    UP-VLA~\textit{[ICML'25]}~\cite{zhang2025up} 
    & 27\% & 1\% & 4\% & 24\% & 0\% & 12\% & 56\% & 2\% & 68\% & 2\% & 26\%\\

    TwinVLA~\textit{[ICLR'26]}~\cite{im2025twinvla}
    & 1\% & 0\% & 0\% & 2\% & 2\% & 4\% & 26\% & 3\% & 55\% & 1\% & 15\%\\

    BagelVLA~\textit{[RSS'26]}~\cite{hu2026bagelvla}
    & 34\% & 5\% & 0\% & 21\% & 2\% & 29\% & 58\% & 21\% & 73\% & 8\% & 30\%\\

    HALO~\textit{[ICML'26]}~\cite{shou2026halo}
    & 28\% & 9\% & 5\% & 33\% & 10\% & 18\% & 64\% & 11\% & 66\% & 21\% & 27\%\\
    
    \midrule
    \rowcolor[HTML]{EFE9F7} 
    \textbf{UniMPA} 
    & \textbf{57\%} & \textbf{19\%} & \textbf{38\%} & \textbf{59\%} & \textbf{37\%} & \textbf{49\%} & \textbf{67\%} & \textbf{22\%} & \textbf{95\%} & \textbf{24\%} & \textbf{34\%} \\
    \bottomrule
    
    \end{tabular}
}
\vspace{-3pt}

\end{table*}

==> authors.tex <==
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi
% \bibliographystyle{IEEEtran}
% \bibliography{main} 

\vspace{-20pt}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author-Figures/LW.jpg}}]
{Wei Li} received his M.Eng. degree in Electronic Information from the University of Chinese Academy of Sciences in 2024 and his B.Eng. degree in Information Engineering from Jilin University in 2021. He is currently a Ph.D. student at Harbin Institute of Technology (Shenzhen). His research interests include computer vision, multimodal large models, and embodied intelligence. 
\end{IEEEbiography}



\vspace{-30pt}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author-Figures/SR.png}}]
{Rui Shao} is currently a professor with Harbin Institute of Technology (Shenzhen). He received his B.Eng. and Ph.D. degree from University of Electronic Science and Technology of China in 2015 and Hong Kong Baptist University in 2021, respectively. His research interests lie primarily in multimodal learning and computer vision. He has published more than 50 papers in top journals and conferences, such as TPAMI, IJCV, CVPR, ICCV. He serves as a reviewer for many top journals and conferences, including TPAMI, IJCV, CVPR, ICCV. He serves as an Area Chair of CVPR, ICPR, BMVC, Senior Program Committee of AAAI and Panel Chairs of ICMR.
\end{IEEEbiography}



\vspace{-30pt}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author-Figures/HJ.jpg}}]
{Jie He } is currently pursuing the B.Eng. degree in Computer Science and Technology at Harbin Institute of Technology (Shenzhen). His research interests include vision-language-action models, embodied intelligence, robotic manipulation, and world models.
\end{IEEEbiography}


\vspace{-30pt}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author-Figures/ZLS.png}}]
{Lingsen Zhang} received his B.Eng. degree in Computer Science and Technology from Harbin Institute of Technology (Shenzhen), Shenzhen, China, in 2025. He is currently pursuing the M.Eng. degree in Computer Technology at Harbin Institute of Technology (Shenzhen). His research interests include computer vision, multimodal large language models, and embodied intelligence.
\end{IEEEbiography}


\vspace{-20pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author-Figures/LZW.jpg}}]
{Ziwei Liu} is currently an Assistant Professor at Nanyang Technological University (NTU). Previously, he was a senior research fellow at the Chinese University of Hong Kong and a postdoctoral researcher at the University of California, Berkeley. Ziwei received his Ph.D. from the Chinese University of Hong Kong in 2017. His research revolves around computer vision/graphics, machine learning, and robotics. He has published extensively on top-tier conferences and journals in relevant fields, including CVPR, ICCV, ECCV, NeurIPS, IROS, SIGGRAPH, TOG, and TPAMI. He is the recipient of the Microsoft Young Fellowship, Hong Kong PhD Fellowship, ICCV Young Researcher Award, and HKSTP best paper award.
\end{IEEEbiography}


\vspace{-15pt}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author-Figures/NLQ.png}}]
{Liqiang Nie}, IAPR Fellow, is currently the dean with the School of Computer Science and Technology, Harbin Institute of Technology (Shenzhen campus). He received his B.Eng. and Ph.D. degree from Xi'an Jiaotong University and National University of Singapore (NUS), respectively. His research interests lie primarily in multimedia content analysis and information retrieval. Dr. Nie has co-/authored more than 100 CCF-A papers and 5 books, with 24k Google Scholar citations. He is an AE of IEEE TKDE, IEEE TMM, IEEE TCSVT, ACM ToMM, and Information Science. Meanwhile, he is the regular area chair or SPC of ACM MM, NeurIPS, ICML and ICME. He is a member of ICME steering committee. He has received many awards, like SIGMM emerging leaders in 2018, ACM MM and SIGIR best paper honorable mention in 2019, SIGMM rising star in 2020, MIT TR35 China 2020, DAMO Academy Young Fellow in 2020, SIGIR best student paper in 2021, ACM MM best paper award in 2022, AI’s 10 to Watch in 2022. Some of his research outputs have been integrated into the products of some listed companies. 
\end{IEEEbiography}
